InferF: Declarative Factorization of AI/ML Inferences over Joins

Real-world AI/ML workflows often apply inference computations to feature vectors joined from multiple datasets. To avoid the redundant AI/ML computations caused by repeated data records in the join's output, factorized ML has been proposed to decompose ML computations into sub-computations to be executed on each normalized dataset. However, there is insufficient discussion on how factorized ML could impact AI/ML inference over multi-way joins. To address the limitations, we propose a novel declarative InferF system, focusing on the factorization of arbitrary inference workflows represented as analyzable expressions over the multi-way joins. We formalize our problem to flexibly push down partial factorized computations to qualified nodes in the join tree to minimize the overall inference computation and join costs and propose two algorithms to resolve the problem: (1) a greedy algorithm based on a per-node cost function that estimates the influence on overall latency if a subset of factorized computations is pushed to a node, and (2) a genetic algorithm for iteratively enumerating and evaluating promising factorization plans. We implement InferF on Velox, an open-sourced database engine from Meta, evaluate it on real-world datasets, observed up to 11.3x speedups, and systematically summarized the factors that determine when factorized ML can benefit AI/ML inference workflows.

==> revision-plan.tex <==
%\section*{\centering Revision Plan}
%\title{Revision Plan}
%\section* {Revision Plan}
This document outlines our response to each review comment and question, as well as the changes we intend to make in a revision. It ends with a timeline for completing all proposed revision actions.

\vspace{-15pt}
\subsection*{Response to Reviewer 1}
We thank Reviewer \#1 for their helpful feedback and recognize that we need to better clarify the scope and contributions of our work. 
\vspace{3pt}
\noindent
\phantomsection\label{target:R1O1}
\underline{\textbf{R1O1} IID issues of training ML models over relational data}:
As detailed in the \textit{Clarification of Misunderstanding}, our work focuses on optimizing inference of pretrained models rather than training. Our work builds upon the practical performance needs of prominent systems that apply pretrained ML models to relational data.

\textbf{$\bullet$ Actions.}
We will add a paragraph to the introduction and related work sections that clearly states this work focuses on inference and does not address model training.

We will add a Future Work paragraph to Section 7, to discuss the papers mentioned by R1, and recommend the examination of the limitations of using models trained on IID data for relational data inference as a potential future direction. 

\vspace{3pt}
\noindent
\phantomsection\label{target:R1O2}
\underline{\textbf{R1O2} Contributions:}
As detailed in our \textit{Clarification of Misunderstanding}, our contributions encompass both theoretical and systems aspects, including problem formalization, novel algorithm design, and systems design and engineering for end-to-end inference factorization over multi-way joins. 

\textbf{$\bullet$ Actions.} To emphasize the novel contributions of \InferF, we will add a summary table to the Related Works section, comparing it to existing systems (LMFAO, MADlib, Morpheus, etc.) across dimensions such as: Target Workload (inference vs. training), Inference Workflows Supported (arbitrary/specific models), Partial Pushdown Support (full/limited/none), Support for Multi-Way Joins (full/limited/none), and Support for Fuzzy Joins (full/limited/none).


\vspace{3pt}
\noindent
\phantomsection\label{target:R1O3}
\underline{\textbf{R1O3} More precise description of existing works:}
First, there are no factorized ML works that have formally defined and thoroughly explored the partial factorization and push-down problem, which is critical to the inference process. 

Second, while Morpheus~\cite{factorize-la} and FL~\cite{kumar2015learning} rely on heuristics, including the tuple ratio or the feature ratio between fact and dimension tables, to decide whether to apply factorization to a join node, the evaluation of these works is limited to joins over two to three tables. We found their heuristics ineffective in a broad class of scenarios, including (1) fuzzy joins that lack foreign key relationships and (2) multi-way joins where the intermediate join nodes do not follow foreign key relationships. 

Third, distinct from Morpheus~\cite{factorize-la} and FL~\cite{kumar2015learning}, our proposed approaches are formalized for a more general problem that applies to any multi-way joins, encompassing both star-schema joins and fuzzy joins. The decoupling of join order optimization and factorization optimization, as well as the greedy strategy, is proposed to effectively resolve this more general problem.



%\textcolor{blue}{Should we also talk about our own assumptions here?}

\textbf{$\bullet$ Actions.}
We will revise the Introduction to present our discussion of prior methods more precisely, while clarifying the assumptions in our own approach and highlighting how our formalization and algorithms go beyond existing works.

\vspace{3pt}
\noindent
\phantomsection\label{target:R1O4}
\underline{\textbf{R1O4} Simplifying Figure 1:}
This is a great suggestion! We will simplify Figure 1 in the revised version.

\textbf{$\bullet$ Actions.}
We will simplify the workflow used in Figure 1. Some ideas we have now include: (1) In subfigures \textit{a} and \textit{d}, we will highlight only factorizable computations, such as \textit{matMul}, abstracting other operations. (2) We will simplify the query plan in subfigure \textit{d} by removing labels that do not affect the understanding of the figure, such as $e_{proj1}$, $e_{proj2}$, etc.


\vspace{3pt}
\noindent
\phantomsection\label{target:R1O5}
\underline{\textbf{R1O5} New experiments using real-world models:}
 We acknowledge that experimental evaluation with real-world models will strengthen the impact of our work. Please note that the Microsoft customer engagement workload that we mentioned in the introduction is proprietary and not publicly available. Therefore, we have chosen two real-world multi-way join workloads, \textit{Flight} and \textit{Expedia}, which have been used to evaluate realworld systems Microsoft's Raven~\cite{park2022end} and OceanDB's IMBridge@SIGMOD'25, to enhance our evaluation. In these workloads, inferences of decision tree and linear regression models are applied to the output of join queries on the \textit{Expedia} and \textit{Flight} datasets. 

\textbf{$\bullet$ Actions.}
Following the recommendation, we will update the experimental evaluation by adding two new real-world experimental workloads \textit{Flight} and \textit{Expedia} to Section 6.

\subsection*{Response to Reviewer 2}
We sincerely appreciate Reviewer 2's supportive and constructive feedback. We are encouraged by their assessment.

\noindent
\phantomsection\label{target:R2O1}
\underline{\textbf{R2O1} Support for traditional factorized ML techniques:} 
You are correct--the specific optimizations proposed in [49, 48, 22] are not supported in our system.
Our work addresses the inference phase of arbitrary ML models, whereas [49, 48, 22, etc.] focus on the training process for models that represent quadratic feature interactions as a semi-ring or a batch of aggregations. Inference in many AI models does not involve such quadratic feature interactions, making those optimizations less relevant to our setting. 

\textbf{$\bullet$ Actions.}
We will add a clarification to the introduction. 

\vspace{3pt}
\noindent
\phantomsection\label{target:R2O2}
\underline{\textbf{R2O2} Assumptions for models to be supported:}
No, to apply our proposed Greedy and Genetic algorithms, the model does not need to be trained with factorized learning. Theoretically, it can be any pretrained model, as long as the model contains factorizable computations that consume the join outputs. 

To use our \InferF end-to-end system for automatically identifying factorizable computations and applying our algorithms, the pretrained model or inference workflows must first be translated to our proposed intermediate representation (IR). Currently, we support translation from models associated with ONNX IR. However, advanced users can always utilize our IR as a Domain-Specific Language (DSL) to represent the model.

\textbf{$\bullet$ Actions.}
We will add a subsection at the end of Section 5 to discuss the user interfaces and the models supported.

\vspace{3pt}
\noindent
\phantomsection\label{target:R2O3}
\underline{\textbf{R2O3} NP-hardness:}
Our NP-hardness argument is based on a reduction from the Sum Product Optimization (SPO) problem. Specifically, given any instance of SPO with $F =\{(s_1, d_1), …, (s_n, d_n)\}$, we construct a left-deep join tree comprising $n$ nodes. In this construction, each $s_i$ is mapped to the additive inference computational cost at the $i^{th}$ node, and each $d_i$ is mapped to the multiplicative join cost at the same node. This transformation can be carried out in polynomial time, thus establishing the reduction.

\textbf{$\bullet$ Actions.}
We will expand Section 3.1 to present a formal proof.

\vspace{3pt}
\noindent
\phantomsection\label{target:R2O4}
\underline{\textbf{R2O4} Inconsistent cumulative latency plots:}
We apologize for the confusion caused by Figure 5. The difference arises from how cumulative latency is plotted. In the left plot, the cumulative latency begins with the latency of the first query over $2$ tables and accumulates thereafter, whereas in the right plot, it begins with the latency of the first query over $10$ tables.

\textbf{$\bullet$ Actions.}
To remove the ambiguity, we will update Figures 5 and 6 so that the cumulative latency in each right plot continues from the accumulated latency of the corresponding left plot, as illustrated in Figure \ref{fig:optimizer-synthetic-new} (for Figure 5).

\vspace{3pt}
\noindent
\phantomsection\label{target:R2O5}
\underline{\textbf{R2O5} Latency measurement:} 
Yes, reported runtimes include both optimization time and query execution time.

\textbf{$\bullet$ Actions.}
We will clarify this at the beginning of Section 6.3.

\begin{figure}[ht]
\vspace{-5pt}
\centering
\includegraphics[width=0.48\textwidth]{images/eval-split-synthetic-new.pdf}
\caption{\small Cumulative End-to-End Latency Comparison on $50$ Queries over  Datasets Synthesized from Bosch and Epsilon. %\textcolor{blue}{Duplicate x-ticks are omitted for clarity, where empty ticks maintain the same value as the last labeled tick.}
}
\label{fig:optimizer-synthetic-new}
\vspace{-2pt}
\end{figure}

\noindent
\underline{\textbf{Reviewers' minor remarks.}} We agree and will fix all those issues in the revised version.

\vspace{-5pt}
\subsection*{Response to Reviewer 3}

We thank Reviewer 3 for helpful feedback, which highlighted areas where we can improve the clarity of our paper. %We believe that the reviewer's major concerns stem from misunderstandings about our optimization objective and system implementation. 

\vspace{3pt}
\noindent
\phantomsection\label{target:R3O1}
\underline{\textbf{R3O1} CPU costs:} As detailed in our \textit{Clarification of Misunderstandings}, the CPU cost saving comes from (1) eliminating redundant inference sub-computations caused by data duplication introduced by joins; and (2) alleviating join costs by reducing the dimensions of tuples input to join nodes, by applying factorized inference computations to the join's input data. 


\textbf{$\bullet$ Actions.} We will better highlight the benefits of factorized ML in the introduction and reintroduce the pipeline of \textit{factorization} $\Rightarrow$ \textit{pushdown} $\Rightarrow$ \textit{join} $\Rightarrow$ \textit{final aggregation} and the benefits at a high level at the beginning of section 2, assuming the readers may not have fully grasped these from the introduction.


\vspace{3pt}
\noindent
\phantomsection\label{target:R3O2}
\underline{\textbf{R3O2} $s_i$:} As explained in the \textit{Clarification of Misunderstandings}, in Eq. 3, $s_i$ for join node $N_i$ denotes the total computational cost of all factorized operations pushed to $N_i$ for all tuples output from $N_i$.  It represents the cost of performing the factorized inference computations pushed to that node.

\textbf{$\bullet$ Actions.} We will enhance the Introduction section to more explicitly state our optimization goals. In Section 3.1, before introducing Equation 3, we will re-emphasize these objectives. 

\vspace{3pt}
\noindent
\phantomsection\label{target:R3O3}
\underline{\textbf{R3O3} Latency reduction:} As detailed in the \textit{Clarification of Misunderstandings}, \InferF aims to select the optimal factorization/pushdown plan to minimize latency, translated to a weighted sum of (inference) computational and join costs across all join nodes, for a multi-way join. Choosing different factorization and pushdown plans will affect the computational cost of the query, as it determines the total amount of inference computations (i.e., how many computations over redundant records can be eliminated). The plan may also influence the join cost, because the computation pushed down may change the dimensions of the tuples to the next join.

\textbf{$\bullet$ Actions.} We will rewrite Section 3.1 to more clearly state the optimization objective (minimizing latency as a function of inference computation and join costs).

\vspace{3pt}
\noindent
\phantomsection\label{target:R3O4}
\underline{\textbf{R3O4} A bottom-up approach minimizing local output size:} We appreciate your suggestion; as clarified, (1) the reduction of the tuple dimension (width) at an intermediate join node $N_i$, and the reduction of the redundant computation achieved by pushing factorized computation $f_j$ to $N_i$, are determined by different aspects: the tuple width reduction is determined by the feature reduction capability of $f_j$, while the redundancy elimination is determined by $f_j$'s complexity and the input/output cardinality ratio of $N_i$; (2) The approach of minimizing the output size of each join node while traversing the tree in a bottom-up style has the limitation that it does not consider the reduction of duplicate data and redundant inference computations, which contribute a majority of the performance gain.

\textbf{$\bullet$ Actions.} We will add a discussion to Section 4 (Optimization Algorithms) explaining the limitations of a purely local, bottom-up approach focused solely on minimizing output size. 




\vspace{3pt}
\noindent
\phantomsection\label{target:R3O5}
\underline{\textbf{R3O5 and R3O6} Parallelism, pipelining, and batching:} Great question! As we mentioned at the end of Section 5, we implemented our system in Velox. We leveraged Velox's following capabilities: 
%
\textbf{Parallelism.} Velox supports data parallelism by splitting an input table into data splits, and launching a thread over each split.
%
\textbf{Pipelining and Batching.} Velox supports pipelining and batching for avoiding data materialization and reducing virtual function call overhead. It splits the query plan into multiple pipelines, where each pipeline is a sequence of operators that ends with a pipeline breaker. A pipeline breaker must have output materialized, such as shuffling (exchange), writing to a file, and building a hash table (for aggregation or join probing). All operators within the pipeline are fused without data materialization. The processing of one pipeline consists of multiple iterations, where each iteration fetches an input batch of tuples and applies a sequence of vectorized operators to the batch, with the output of the pipeline being materialized by the pipeline breaker. Velox adopts a push-based execution model for scheduling pipelines. Data parallelism and Pipelining are widely supported in DB systems.

\textbf{$\bullet$ Actions.} We will clarify the above at the end of Section 5.

\vspace{3pt}
\noindent
\phantomsection\label{target:R3O7}
\underline{\textbf{R3O7} The case with $x_i = 0$:} 
{\color{red}{
Great catch! We missed a constraint that each factorized subcomputation not pushed to any non-root tree nodes must be computed at the root node.%: $x_{2m-1} = 1, \text{ if } D_{2m-1} \neq \phi$

\textbf{$\bullet$ Actions.} We will revise Section 3.1 to add the new constraint "$\color{red}{x_{2m-1} = 1, \text{ if } D_{2m-1} \neq \phi}$" immediately after Eq 2.}}


%\noindent
%\textbf{Action Item 4-1.} We will correct this statement in Section 8 and explain how our work is distinguished from the mentioned related work by considering accuracy and differential privacy.

\vspace{6pt}
\centering
\textbf{Proposed Timeline for Action Items}

\centering
\small
\begin{tabular}
{ |c|c|  }
 \hline
 & Actions to complete\\
 \hline
%\hyperref[box:R1-Summary]{R1-Summary}&1-2&W1\\
Week1 &\hyperref[target:R1O5]{R1O5} (New Experiments), \hyperref[target:R1O4]{R1O4} (Fig. 1), \hyperref[target:R2O4]{R2O4} \& \hyperref[target:R2O5]{R2O5} (Sec. 6)  \\
Week2 &Sec. 3-5: \hyperref[target:R2O2]{R2O2},   \hyperref[target:R2O3]{R2O3}, \hyperref[target:R3O2]{R3O2}, \hyperref[target:R3O3]{R3O3}, \hyperref[target:R3O4]{R3O4}, \hyperref[target:R3O5]{R3O5}, \hyperref[target:R3O6]{R3O6}, \hyperref[target:R3O7]{R3O7}  \\
Week3 &Sec. 1, 2, 7: \hyperref[target:R1O1]{R1O1}, \hyperref[target:R1O2]{R1O2}, \hyperref[target:R1O13]{R1O3}, \hyperref[target:R2O1]{R2O1}, \hyperref[target:R3O1]{R3O1}, Minor remarks\\
Week4 & Refinement and proof-reading\\
 \hline
\end{tabular}
